Small Language Models Learn Enhanced Reasoning Skills from Medical Textbooks

While recent advancements in commercial large language models (LM) have shown promising results in medical tasks, their closed-source nature poses significant privacy and security concerns, hindering their widespread use in the medical field. Despite efforts to create open-source models, their limited parameters often result in insufficient multi-step reasoning capabilities required for solving complex medical problems. To address this, we introduce Meerkat, a new family of medical AI systems ranging from 7 to 70 billion parameters. The models were trained using our new synthetic dataset consisting of high-quality chain-of-thought reasoning paths sourced from 18 medical textbooks, along with diverse instruction-following datasets. Our systems achieved remarkable accuracy across six medical benchmarks, surpassing the previous best models such as MediTron and BioMistral, and GPT-3.5 by a large margin. Notably, Meerkat-7B surpassed the passing threshold of the United States Medical Licensing Examination (USMLE) for the first time for a 7B-parameter model, while Meerkat-70B outperformed GPT-4 by an average of 1.3%. Additionally, Meerkat-70B correctly diagnosed 21 out of 38 complex clinical cases, outperforming humans' 13.8 and closely matching GPT-4's 21.8. Our systems offered more detailed free-form responses to clinical queries compared to existing small models, approaching the performance level of large commercial models. This significantly narrows the performance gap with large LMs, showcasing its effectiveness in addressing complex medical challenges.

==> tables/ablation.tex <==
\begin{table}[ht]
\caption{
Others include a instruction-tuning dataset (i.e., AlpaCare), two long-form medical QA datasets (i.e., LiveQA and Medication QA), patient-doctor conversations, and clinical note summaries (i.e., MTS and ACI-Bench).
}\label{tab:ablation}
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{MedQA}} & \multirow{2}{*}{\textbf{MedMCQA}} & \multicolumn{3}{c}{\textbf{MMLU-Medical}} \\
\cmidrule(lr){4-6}
& & & \textbf{Prof. Med.} & \textbf{Others} & \textbf{All} \\
\midrule
\multicolumn{6}{l}{In-context Learning (3-shot)} \\
\midrule
LLaMA-2-7B\footnotemark[1] & 35.4$_{\pm 4.3}$ & 36.3$_{\pm 1.4}$ & - & - & 41.4$_{\pm 0.2}$ \\
PMC-LLaMA-7B\footnotemark[1] & 27.8$_{\pm 0.9}$ & 27.4$_{\pm 5.9}$ & - & - & 26.2$_{\pm 1.3}$ \\
MediTron-7B\footnotemark[1] & 37.4$_{\pm 3.3}$ & 36.3$_{\pm 1.4}$ & - & - & 42.3$_{\pm 2.4}$ \\
\midrule
\multicolumn{6}{l}{Supervised Fine-tuning} \\
\midrule
LLaMA-2-7B & 35.4$_{\pm 4.3}$ & 36.3$_{\pm 1.4}$ & - & - & 41.4$_{\pm 0.2}$ \\
PMC-LLaMA-7B & 27.8$_{\pm 0.9}$ & 27.4$_{\pm 5.9}$ & - & - & 26.2$_{\pm 1.3}$ \\
MediTron-7B &  \\
MediTron-7B &  \\
Gemma-7B &  \\
\midrule
\multicolumn{6}{l}{Chain-of-thought Fine-tuning} \\
\midrule
MedQA CoT (w/ humans) & xx.x$_{\pm x.x}$ &  &   \\
\hdashline
MedQA CoT & 54.3$_{\pm1.1}$ & 40.1$_{\pm0.7}$ & 59.4$_{\pm2.0}$ & 50.4$_{\pm0.7}$ & 52.0$_{\pm0.5}$  \\
+ Textbooks & 62.2$_{\pm0.7}$ & 45.3$_{\pm0.8}$ & 69.0$_{\pm1.1}$ & \\
+ medmcqa cot & 63.3$_{\pm1.1}$ & 46.7$_{\pm0.3}$ &  & \\
+ Others & 61.7$_{\pm1.1}$ & 45.7$_{\pm0.7}$ & 70.2$_{\pm2.0}$ & 58.4$_{\pm1.2}$ & 60.5$_{\pm0.8}$  \\
+ Ensemble with choice shuffle & 68.4$_{\pm0.8}$ &  & \\
\bottomrule
\end{tabular}
\footnotetext[1]{The scores are obtained from~\citet{chen2023meditron}.}
\end{table}

==> tables/llm_comparison.tex <==
\begin{table}[t!]
\caption{
asdf
}\label{tab:llm_comparision}
\begin{tabular}{lllrc}
\toprule
\textbf{Model} & \textbf{Initial Weights} & \textbf{Corpus} & \textbf{Release} & \textbf{MedQA} \\
\midrule
PMC-LLaMA-7B~\cite{wu2023pmc} & LLaMA 7B & PMC, Textbooks & Apr 2023 &  \\
LLaMA-2-7B~\cite{touvron2023llama2} & - & & Jul 2023 & 59.1$_{\pm0.9}$ \\
Mistral-7B~\cite{jiang2023mistral} & - & & Oct 2023 & \textbf{63.3}$_{\pm0.5}$ \\
MediTron-7B~\cite{chen2023meditron} & LLaMA 7B & PMC & Nov 2023 & 62.2$_{\pm0.7}$ \\
OLMo-7B~\cite{groeneveld2024olmo} & - & & Feb 2024 & \\
BioMistral-7B~\cite{labrak2024biomistral} & Mistral 7B & PMC & Feb 2024 & 62.7$_{\pm0.4}$ \\
Gemma-7B~\cite{google2024gemma} & - & Unknown & Feb 2024 & 63.1$_{\pm0.3}$ \\
\midrule
Mixtral-8x7B~\cite{jiang2024mixtral} &  & Unknown & Jan 2024 &  \\
\midrule
\end{tabular}
\end{table}


==> tables/mmlu.tex <==
\begin{table}[h!]
\captionsetup{width=\textwidth}
\caption{
Performance of models for six medical subjects in MMLU-Medical~\cite{hendrycks2020measuring}.
Our Meerkat-7B model showed the highest performance among 7B models and generally performed comparably to GPT-3.5 and Clinical Camel-70B. 
The scores for GPT-4 and GPT-3.5 were sourced from the study by~\citet{nori2023capabilities}, while the scores for 70B models were taken from the study by~\citet{chen2023meditron}.
``Ens'' indicates that the scores were obtained using ensemble methods.
``Cliniq K'': Clinical knowledge. 
``Med Gen'': Medical genetics.
``Anat'': Anatomy.
``Pro Med'': Professional medicine.
``C Bio'': College biology.
``C Med'': College medicine.
}\label{tab:mmlu}
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} & \textbf{Cliniq K} & \textbf{Med Gen} & \textbf{Anat} & \textbf{Pro Med} & \textbf{C Bio} & \textbf{C Med} \\
\midrule
\multicolumn{3}{l}{\textbf{Closed-source Model}} \\
\midrule
GPT-4 (5-shot) & \underline{86.4} & \underline{92.0} & \underline{80.0} & \underline{93.8} & \underline{93.8} & \underline{76.3}
 \\
GPT-3.5 (5-shot) & 68.7 & 68.0 & 60.7 & 69.9 & 72.9 & 63.6 \\
%Flan-PaLM & \underline{77.0} & \underline{70.0} & 65.2 & \underline{83.8} & 87.5 & 69.9 \\
%Flan-PaLM (Ens) & 67.6 & 57.6 & \underline{79.2} & 80.4 & \underline{88.9} & \underline{76.3} \\
\midrule
%Med-Alpaca-13B & 27.9 & 24.2 & 25.3 & 32.4 & 30.4 & 26.5 \\
%PMC-LLaMA-13B & 59.2 & 59.0 & 45.2 & 55.1 & 51.4 & 52.6 \\
\multicolumn{3}{l}{\textbf{Open-source Model (70B)}} \\
\midrule
Clinical Camel-70B~\cite{toma2023clinical} & 65.1 & 62.6 & 56.0 & 71.6 & 69.2 & 56.3 \\
LLaMA-2-70B (Ens)~\cite{touvron2023llama2} & {76.5} & 81.1 & {70.9} & {82.3} & \underline{90.9} & {72.1}  \\
MediTron-70B (Ens)~\cite{chen2023meditron} & 75.5 & {85.9} & 69.4 & {82.3} & 86.7 & 68.0 \\
Meerkat-70B (\textbf{Ours}) & \underline{87.2} & \underline{88.2} & \underline{84.4} & \underline{87.2} & {87.9} & \underline{86.6} \\

\midrule
\multicolumn{3}{l}{\textbf{Open-source Model ($<$ 10B)}} \\
\midrule
%PMC-LLaMA-7B$^\ast$~\cite{wu2023pmc} & 63.3 & 69.7 & 55.2 & 57.6 & 57.3 & 55.8 \\
%LLaMA-2-7B$^\ast$~\cite{touvron2023llama2} & 59.8 & 71.8 & 48.5 & 53.5 & 53.1 & 50.0 \\
%Mistral-7B-Instruct$^\ast$~\cite{jiang2023mistral} & 57.9 & 56.6 & 44.0 & 55.7 & 58.7 & 52.3 \\
MediTron-7B~\cite{chen2023meditron} & 57.7 & 63.8 & 56.9 & 56.0 & 57.1 & 48.9 \\
BioMistral-7B~\cite{labrak2024biomistral} & 59.9 & 64.0 & 56.5 & 60.4 & {59.0} & 54.7 \\
Meerkat-7B (\textbf{Ours}) & {71.6} & {74.8} & {63.2} & \underline{77.3} & {70.8} & {65.2} \\
Meerkat-8B (\textbf{Ours}) & \underline{74.3} & \underline{76.7} & \underline{74.8} & {75.3} & \underline{76.1} & \underline{74.3} \\
\bottomrule
\end{tabular}
\end{table}
